Nonparametric Variable Screening with Optimal Decision Stumps

Decision trees and their ensembles are endowed with a rich set of diagnostic tools for ranking and screening variables in a predictive model. Despite the widespread use of tree based variable importance measures, pinning down their theoretical properties has been challenging and therefore largely unexplored. To address this gap between theory and practice, we derive finite sample performance guarantees for variable selection in nonparametric models using a single-level CART decision tree (a decision stump). Under standard operating assumptions in variable screening literature, we find that the marginal signal strength of each variable and ambient dimensionality can be considerably weaker and higher, respectively, than state-of-the-art nonparametric variable selection methods. Furthermore, unlike previous marginal screening methods that attempt to directly estimate each marginal projection via a truncated basis expansion, the fitted model used here is a simple, parsimonious decision stump, thereby eliminating the need for tuning the number of basis terms. Thus, surprisingly, even though decision stumps are highly inaccurate for estimation purposes, they can still be used to perform consistent model selection.

==> conclusion.tex <==
In this paper, we developed a theoretically rigorous approach for variable selection based on decision trees. The underlying approach is simple, intuitive, and interpretable—we test whether a variable is relevant/irrelevant by fitting a decision stump to that variable and then determining how much it explains the variance of the response variable. Despite its simplicity, SDI performs favorably for nonparametric models with an additive structure. Due to the parsimony of the model, there is also no need to perform bandwidth selection or calibrate other tuning parameters (e.g., penalty or degree of basis expansion). 

On the other hand, we have sacrificed generality for analytical tractability. That is, decision stumps are poor at capturing non-additive effects and, therefore, an importance measure built from a multi-level decision tree (such as MDI) may more appropriate for certain models. However, the presence of multi-level splits adds an additional layer of complexity to the analysis that, at the moment, we do not know how to overcome. While out of the scope of the present paper, we view this as an important problem for future investigation. It is our hope that the tools in this paper can be used by other scholars for such an end.

